Discriminatory Expressions to Produce Interpretable Models in Short Documents

Social Networking Sites (SNS) are one of the most important ways of communication. In particular, microblogging sites are being used as analysis avenues due to their peculiarities (promptness, short texts...). There are countless researches that use SNS in novel manners, but machine learning has focused mainly in classification performance rather than interpretability and/or other goodness metrics. Thus, state-of-the-art models are black boxes that should not be used to solve problems that may have a social impact. When the problem requires transparency, it is necessary to build interpretable pipelines. Although the classifier may be interpretable, resulting models are too complex to be considered comprehensible, making it impossible for humans to understand the actual decisions. This paper presents a feature selection mechanism that is able to improve comprehensibility by using less but more meaningful features while achieving good performance in microblogging contexts where interpretability is mandatory. Moreover, we present a ranking method to evaluate features in terms of statistical relevance and bias. We conducted exhaustive tests with five different datasets in order to evaluate classification performance, generalisation capacity and complexity of the model. Results show that our proposal is better and the most stable one in terms of accuracy, generalisation and comprehensibility.

==> sections/annexcomplementary.tex <==
We present in this section complementary tables~\ref{tab:complementary1}, \ref{tab:complementary2}, \ref{tab:complementary3}, \ref{tab:complementary4}, \ref{tab:complementary5} and \ref{tab:complementary6} that show in-depth performance and stability results.

\begin{table}
    \centering
    \caption{Classification performance of our proposal (DE) against the rest of the selected methods measured with accuracy (acc), precision (pre), recall (rec), $f1$-score (f1) and area-under-curve ROC (rocauc) when training with 9 features. Results show that DE performs better in 3 out of 4 datasets.}
    \label{tab:complementary1}
    \begin{tabular}{lrrrrr}
    \toprule
    FS method &    acc &    pre &    rec &     f1 &  rocauc \\
    \midrule
    \textbf{airlines dataset}\\
    \hspace{2mm}CHI2 & 0.8745 & 0.6364 & 0.5251 & 0.5696 &  0.7334 \\
    \hspace{2mm}DE & 0.8664 & 0.6308 & 0.4640 & 0.5295 &  0.7039 \\
    \hspace{2mm}ECE & 0.8696 & 0.6694 & 0.3795 & 0.4824 &  0.6717 \\
    \hspace{2mm}f-ANOVA & 0.8771 & 0.6456 & 0.5406 & 0.5835 &  0.7413 \\
    \hspace{2mm}GSS & 0.8686 & 0.6450 & 0.4816 & 0.5379 &  0.7123 \\
    \hspace{2mm}IG & 0.8792 & 0.6537 & 0.5383 & \textbf{0.5869} &  0.7415 \\
    \hspace{2mm}MI & 0.8786 & 0.6562 & 0.5257 & 0.5802 &  0.7361 \\
    \hspace{2mm}OR & 0.8679 & 0.6488 & 0.4287 & 0.5113 &  0.6906 \\
    \textbf{gender dataset}\\
    \hspace{2mm}CHI2 & 0.5361 & 0.4954 & 0.6805 & 0.5099 &  0.5417 \\
    \hspace{2mm}DE & 0.5704 & 0.5401 & 0.7084 & \textbf{0.6100} &  0.5759 \\
    \hspace{2mm}ECE & 0.5430 & 0.5073 & 0.7293 & 0.5706 &  0.5492 \\
    \hspace{2mm}f-ANOVA & 0.5478 & 0.5153 & 0.7369 & 0.5685 &  0.5553 \\
    \hspace{2mm}GSS & 0.5282 & 0.5636 & 0.2052 & 0.2436 &  0.5157 \\
    \hspace{2mm}IG & 0.5372 & 0.5125 & 0.6883 & 0.5232 &  0.5429 \\
    \hspace{2mm}MI & 0.5360 & 0.5022 & 0.6842 & 0.5176 &  0.5416 \\
    \hspace{2mm}OR & 0.5343 & 0.5051 & 0.6631 & 0.5251 &  0.5386 \\
    \textbf{imdb dataset}\\
    \hspace{2mm}CHI2 & 0.5792 & 0.7027 & 0.5326 & 0.4899 &  0.5829 \\
    \hspace{2mm}DE & 0.6205 & 0.6748 & 0.5447 & \textbf{0.5790} &  0.6216 \\
    \hspace{2mm}ECE & 0.5505 & 0.5781 & 0.4160 & 0.4635 &  0.5494 \\
    \hspace{2mm}f-ANOVA & 0.5825 & 0.6567 & 0.6761 & 0.5598 &  0.5882 \\
    \hspace{2mm}GSS & 0.5885 & 0.6927 & 0.4466 & 0.4989 &  0.5922 \\
    \hspace{2mm}IG & 0.5852 & 0.7247 & 0.5081 & 0.4933 &  0.5894 \\
    \hspace{2mm}MI & 0.5885 & 0.7319 & 0.5023 & 0.4874 &  0.5919 \\
    \hspace{2mm}OR & 0.5725 & 0.6311 & 0.4234 & 0.4825 &  0.5737 \\
    \textbf{tass dataset}\\
    \hspace{2mm}CHI2 & 0.6780 & 0.7735 & 0.3755 & 0.4729 &  0.6274 \\
    \hspace{2mm}DE & 0.6901 & 0.6779 & 0.4299 & \textbf{0.5255} &  0.6467 \\
    \hspace{2mm}ECE & 0.6067 & 0.5907 & 0.2251 & 0.2987 &  0.5433 \\
    \hspace{2mm}f-ANOVA & 0.6930 & 0.7985 & 0.3438 & 0.4677 &  0.6340 \\
    \hspace{2mm}GSS & 0.6594 & 0.7222 & 0.4005 & 0.4722 &  0.6153 \\
    \hspace{2mm}IG & 0.6974 & 0.8062 & 0.3217 & 0.4583 &  0.6346 \\
    \hspace{2mm}MI & 0.6945 & 0.8084 & 0.3433 & 0.4685 &  0.6352 \\
    \hspace{2mm}OR & 0.6376 & 0.6158 & 0.2958 & 0.3882 &  0.5804 \\
    \bottomrule
    \end{tabular}
\end{table}

\begin{table}
    \centering
    \caption{Performance dispersion of our proposal (DE) against the rest of the selected methods measured with range, interquartile range (IQR), standard deviation (STD) and coefficient of variation (CV) when training with 9 features. Results show that DE performs better in 2 out of 4 datasets.}
    \label{tab:complementary2}
    \begin{tabular}{lrrrr}
    \toprule
    FS method &  range &    IQR &    STD &  CV (\%) \\
    \midrule
    \textbf{airlines dataset}\\
    \hspace{2mm}CHI2 & 0.2835 & 0.0290 & 0.0671 & 11.7734 \\
    \hspace{2mm}DE & 0.1833 & 0.1018 & 0.0603 & 11.3899 \\
    \hspace{2mm}ECE & 0.2158 & 0.0185 & 0.0478 &  9.9008 \\
    \hspace{2mm}f-ANOVA & 0.2496 & 0.0242 & 0.0511 &  8.7641 \\
    \hspace{2mm}GSS & 0.1740 & 0.0986 & 0.0570 & 10.6049 \\
    \hspace{2mm}IG & 0.2306 & 0.0364 & 0.0501 &  8.5442 \\
    \hspace{2mm}MI & 0.2273 & 0.0315 & 0.0474 &  \textbf{8.1757} \\
    \hspace{2mm}OR & 0.2366 & 0.0639 & 0.0608 & 11.8858 \\
    \textbf{gender dataset}\\
    \hspace{2mm}CHI2 & 0.6253 & 0.1494 & 0.2537 & 49.7470 \\
    \hspace{2mm}DE & 0.2185 & 0.0124 & 0.0471 &  \textbf{7.7200} \\
    \hspace{2mm}ECE & 0.5159 & 0.0188 & 0.1741 & 30.5157 \\
    \hspace{2mm}f-ANOVA & 0.5760 & 0.0159 & 0.1939 & 34.1072 \\
    \hspace{2mm}GSS & 0.4959 & 0.0260 & 0.1373 & 56.3815 \\
    \hspace{2mm}IG & 0.5460 & 0.1397 & 0.2286 & 43.6941 \\
    \hspace{2mm}MI & 0.5921 & 0.1404 & 0.2384 & 46.0551 \\
    \hspace{2mm}OR & 0.4917 & 0.1248 & 0.2024 & 38.5512 \\
    \textbf{imdb dataset}\\
    \hspace{2mm}CHI2 & 0.4921 & 0.3695 & 0.1849 & 37.7442 \\
    \hspace{2mm}DE & 0.2283 & 0.0722 & 0.0618 & \textbf{10.6673} \\
    \hspace{2mm}ECE & 0.3600 & 0.1852 & 0.1086 & 23.4350 \\
    \hspace{2mm}f-ANOVA & 0.4719 & 0.3198 & 0.1813 & 32.3765 \\
    \hspace{2mm}GSS & 0.2556 & 0.1483 & 0.0867 & 17.3774 \\
    \hspace{2mm}IG & 0.4180 & 0.3076 & 0.1551 & 31.4443 \\
    \hspace{2mm}MI & 0.4132 & 0.3603 & 0.1691 & 34.7056 \\
    \hspace{2mm}OR & 0.3127 & 0.1125 & 0.0884 & 18.3206 \\
    \textbf{tass dataset}\\
    \hspace{2mm}CHI2 & 0.1926 & 0.0275 & 0.0386 &  8.1571 \\
    \hspace{2mm}DE & 0.1478 & 0.0558 & 0.0360 &  6.8562 \\
    \hspace{2mm}ECE & 0.4576 & 0.0381 & 0.0880 & 29.4679 \\
    \hspace{2mm}f-ANOVA & 0.1692 & 0.0346 & 0.0322 &  6.8889 \\
    \hspace{2mm}GSS & 0.2002 & 0.0716 & 0.0492 & 10.4178 \\
    \hspace{2mm}IG & 0.1029 & 0.0576 & 0.0298 &  \textbf{6.5040} \\
    \hspace{2mm}MI & 0.1725 & 0.0346 & 0.0324 &  6.9091 \\
    \hspace{2mm}OR & 0.3455 & 0.1114 & 0.1015 & 26.1393 \\
    \bottomrule
    \end{tabular}
\end{table}

\begin{table*}
    \centering
    \caption{Classification performance of a deep neural network using ELMo embeddings measured with accuracy (acc), precision (pre), recall (rec), $f1$-score (f1) and area-under-curve ROC (rocauc) without limiting the number of features.}
    \label{tab:complementary3}
    \begin{tabular}{lrrrrrrrrrr}
    \toprule
    {} & \multicolumn{2}{c}{acc} & \multicolumn{2}{c}{pre} & \multicolumn{2}{c}{rec} & \multicolumn{2}{c}{f1} & \multicolumn{2}{c}{rocauc} \\
    {} &   mean &    std &   mean &    std &   mean &    std &   mean &    std &   mean &    std \\
    dataset      &        &        &        &        &        &        &        &        &        &        \\
    \midrule
    airlines & 0.8926 & 0.0064 & 0.7757 & 0.0860 & 0.5037 & 0.1487 & 0.5915 & 0.0888 & 0.7358 & 0.0636 \\
    gender   & 0.5893 & 0.0378 & 0.6528 & 0.0845 & 0.3647 & 0.1727 & 0.4376 & 0.1530 & 0.5808 & 0.0387 \\
    imdb     & 0.7020 & 0.0893 & 0.6992 & 0.1518 & 0.8328 & 0.1701 & 0.7355 & 0.0667 & 0.7138 & 0.0799 \\
    s140.csv     & 0.7313 & 0.0025 & 0.7249 & 0.0185 & 0.7483 & 0.0449 & 0.7353 & 0.0136 & 0.7312 & 0.0025 \\
    tass     & 0.5589 & 0.1094 & 0.6429 & 0.2306 & 0.4950 & 0.4763 & 0.3677 & 0.2659 & 0.5436 & 0.0459 \\
    \bottomrule
    \end{tabular}
\end{table*}


\begin{table*}
    \centering
    \caption{Classification performance against $k$-nearest neighbours (kNN) complexity for each dataset and feature selection method. The lower the number of neighbours is and the higher the $f1$-score, the better.}
    \label{tab:complementary4}
    \begin{tabular}{lrrrrr|r}
    \toprule
    {} & \multicolumn{5}{c}{$f1$-score} & \\
    \hspace{7mm}no. of neighbours &     5  &     7  &     9  &     10 &     25 & $\sum\frac{f1}{k}$ \\
    FS method &        &        &        &        &        &        \\
    \midrule
    \textbf{airlines dataset}\\
    \hspace{2mm}CHI2 & 0.2653 & 0.2763 & 0.3108 & 0.2638 & 0.5918    & 0.1771 \\
    \hspace{2mm}DE & 0.5608 & 0.5604 & 0.5661 & 0.2455 & 0.5688      & 0.3024 \\
    \hspace{2mm}ECE & 0.3582 & 0.3902 & 0.4426 & 0.4264 & 0.5045     & 0.2394 \\
    \hspace{2mm}f-ANOVA & 0.3468 & 0.5773 & 0.5740 & 0.5698 & 0.5970 & 0.2965 \\
    \hspace{2mm}GSS & 0.5370 & 0.5436 & 0.5359 & 0.5157 & 0.5833     & 0.3195 \\
    \hspace{2mm}IG & 0.6000 & 0.6164 & 0.5931 & 0.5869 & 0.5744      & \textbf{0.3556} \\
    \hspace{2mm}MI & 0.6000 & 0.6164 & 0.5931 & 0.5869 & 0.5744      & \textbf{0.3556} \\
    \hspace{2mm}OR & 0.5335 & 0.5203 & 0.4805 & 0.4581 & 0.4323      & 0.2975 \\
    \textbf{gender dataset} \\                                         
    \hspace{2mm}CHI2 & 0.6425 & 0.6432 & 0.6455 & 0.6447 & 0.6519    & \textbf{0.3827} \\
    \hspace{2mm}DE & 0.6451 & 0.6248 & 0.6452 & 0.1281 & 0.6474      & 0.3287 \\
    \hspace{2mm}ECE & 0.6157 & 0.1178 & 0.1181 & 0.1029 & 0.1695     & 0.1702 \\
    \hspace{2mm}f-ANOVA & 0.6390 & 0.6374 & 0.6324 & 0.6335 & 0.6348 & 0.3779 \\
    \hspace{2mm}GSS & 0.1579 & 0.1445 & 0.1448 & 0.1258 & 0.1883     & 0.0884 \\
    \hspace{2mm}IG & 0.6375 & 0.6425 & 0.6415 & 0.6403 & 0.6382      & 0.3801 \\
    \hspace{2mm}MI & 0.1532 & 0.1706 & 0.1508 & 0.0940 & 0.1350      & 0.0866 \\
    \hspace{2mm}OR & 0.6452 & 0.6302 & 0.6282 & 0.6280 & 0.6340      & 0.3770 \\
    \textbf{imdb dataset}\\                                            
    \hspace{2mm}CHI2 & 0.6763 & 0.6763 & 0.6763 & 0.4160 & 0.4160    & 0.3652 \\
    \hspace{2mm}DE & 0.6966 & 0.6966 & 0.6966 & 0.6966 & 0.6966      & \textbf{0.4138} \\
    \hspace{2mm}ECE & 0.6116 & 0.6160 & 0.6213 & 0.3016 & 0.4354     & 0.3269 \\
    \hspace{2mm}f-ANOVA & 0.6788 & 0.6788 & 0.6791 & 0.6791 & 0.3902 & 0.3917 \\
    \hspace{2mm}GSS & 0.6577 & 0.6577 & 0.6577 & 0.5294 & 0.5294     & 0.3727 \\
    \hspace{2mm}IG & 0.6788 & 0.6840 & 0.6840 & 0.4733 & 0.4733      & 0.3757 \\
    \hspace{2mm}MI & 0.6764 & 0.6764 & 0.6764 & 0.3902 & 0.6764      & 0.3731 \\
    \hspace{2mm}OR & 0.6071 & 0.5442 & 0.5616 & 0.4818 & 0.5478      & 0.3317 \\
    \textbf{tass dataset}\\                                            
    \hspace{2mm}CHI2 & 0.4522 & 0.4522 & 0.4814 & 0.4522 & 0.4814    & 0.2730 \\
    \hspace{2mm}DE & 0.3747 & 0.3747 & 0.3730 & 0.3762 & 0.3762      & 0.2226 \\
    \hspace{2mm}ECE & 0.4370 & 0.3993 & 0.4007 & 0.3474 & 0.3789     & 0.2389 \\
    \hspace{2mm}f-ANOVA & 0.4496 & 0.4062 & 0.4062 & 0.4062 & 0.4010 & 0.2497 \\
    \hspace{2mm}GSS & 0.3913 & 0.3656 & 0.4666 & 0.4238 & 0.4169     & 0.2414 \\
    \hspace{2mm}IG & 0.5428 & 0.5657 & 0.4554 & 0.4560 & 0.4547      & \textbf{0.3038} \\
    \hspace{2mm}MI & 0.4470 & 0.4489 & 0.4503 & 0.4484 & 0.4475      & 0.2663 \\
    \hspace{2mm}OR & 0.4520 & 0.4225 & 0.4208 & 0.3675 & 0.4236      & 0.2512 \\
    \bottomrule
    \end{tabular}
\end{table*}

\begin{table*}[tbp]
    \centering
    \caption{Performance and complexity measures of DT-based models for each dataset. Number of leaves (rules) and path length (clauses) can be used to compare how comprehensible are the models that result from training with different feature sets. Our proposal is within the best of them and it produce the only feature set that can manage to keep a good classification performance while maintaining a simple model in the gender classification task.}
    \label{tab:complementary5}
    \begin{tabular}{lrrrr|r}
    \toprule
    FS method &     f1 &  rules &  clauses & complexity & compr. rate \\
    \midrule
    \textbf{airlines dataset}\\
    \hspace{2mm}CHI2 & 0.5981 &      34 &  7.4706 &      7.5901 &            \textbf{ 7.8796} \\
    \hspace{2mm}DE & 0.5698 &      41 &  7.2683 &      8.6638 &             6.5766 \\
    \hspace{2mm}ECE & 0.5026 &      69 &  9.1159 &     22.9357 &             2.1912 \\
    \hspace{2mm}f-ANOVA & 0.6063 &      44 &  7.6136 &     10.2023 &             5.9430 \\
    \hspace{2mm}GSS & 0.5821 &      49 &  7.4082 &     10.7567 &             5.4111 \\
    \hspace{2mm}IG & 0.6016 &      47 &  7.6383 &     10.9686 &             5.4845 \\
    \hspace{2mm}MI & 0.6016 &      47 &  7.6383 &     10.9686 &             5.4845 \\
    \hspace{2mm}OR & 0.5515 &      92 &  9.0543 &     30.1691 &             1.8280 \\
    \textbf{gender dataset}\\
    \hspace{2mm}CHI2 & 0.6429 &     309 & 13.7799 &    234.6999 &             0.2739 \\
    \hspace{2mm}DE & 0.6444 &      28 &  6.5000 &      4.7320 &            \textbf{13.6171} \\
    \hspace{2mm}ECE & 0.6328 &     371 & 13.7278 &    279.6620 &             0.2263 \\
    \hspace{2mm}f-ANOVA & 0.6381 &     234 & 13.0684 &    159.8524 &             0.3992 \\
    \hspace{2mm}GSS & 0.1833 &      48 &  8.5417 &     14.0083 &             1.3087 \\
    \hspace{2mm}IG & 0.6423 &     311 & 13.3698 &    222.3661 &             0.2889 \\
    \hspace{2mm}MI & 0.6421 &     302 & 13.1623 &    209.2798 &             0.3068 \\
    \hspace{2mm}OR & 0.6356 &     333 & 13.0541 &    226.9839 &             0.2800 \\
    \textbf{imdb dataset}\\
    \hspace{2mm}CHI2 & 0.6763 &      15 &  6.6667 &      2.6667 &            25.3597 \\
    \hspace{2mm}DE & 0.6966 &      16 &  6.7500 &      2.9160 &            23.8899 \\
    \hspace{2mm}ECE & 0.4082 &      44 & 10.0227 &     17.6801 &             2.3086 \\
    \hspace{2mm}f-ANOVA & 0.6791 &      14 &  6.5000 &      2.3660 &            28.7026 \\
    \hspace{2mm}GSS & 0.5976 &      17 &  7.1176 &      3.4449 &            17.3460 \\
    \hspace{2mm}IG & 0.6889 &      16 &  6.5000 &      2.7040 &            25.4767 \\
    \hspace{2mm}MI & 0.6764 &      11 &  5.4545 &      1.3091 &            \textbf{51.6667} \\
    \hspace{2mm}OR & 0.5385 &      36 &  8.0000 &      9.2160 &             5.8427 \\
    \textbf{tass dataset}\\
    \hspace{2mm}CHI2 & 0.4807 &      23 &  6.8261 &      4.2868 &            \textbf{11.2146} \\
    \hspace{2mm}DE & 0.3735 &      24 &  6.7083 &      4.3202 &             8.6457 \\
    \hspace{2mm}ECE & 0.3055 &     901 & 14.0954 &    716.0488 &             0.0427 \\
    \hspace{2mm}f-ANOVA & 0.4520 &      23 &  7.1739 &      4.7348 &             9.5465 \\
    \hspace{2mm}GSS & 0.4316 &      36 &  8.3611 &     10.0668 &             4.2870 \\
    \hspace{2mm}IG & 0.4877 &      25 &  7.2800 &      5.2998 &             9.2020 \\
    \hspace{2mm}MI & 0.4509 &      22 &  6.9091 &      4.2007 &            10.7334 \\
    \hspace{2mm}OR & 0.3414 &     834 & 13.4233 &    601.0936 &             0.0568 \\
    \bottomrule
    \end{tabular}
\end{table*}

\begin{table*}
    \centering
    \caption{Performance and complexity measures of RF-based models for each dataset when training with 5 trees. Number of leaves (rules) and path length (clauses) can be used to compare how comprehensible are the models that result from training with different features selection mechanisms.}
    \label{tab:complementary6}
    \begin{tabular}{lrrrr|r}
    \toprule
    FS method &     f1 &   rules &  clauses &  complexity &  compr. rate \\
    \midrule
    \textbf{airlines dataset}\\
    \hspace{2mm}CHI2 & 0.6116 &  58.2000 &  8.2904 &     16.0004 &             \textbf{3.8222} \\
    \hspace{2mm}DE & 0.5691 &  65.8000 &  8.1672 &     17.5561 &             3.2417 \\
    \hspace{2mm}ECE & 0.5057 & 160.2000 &  9.8588 &     62.2831 &             0.8120 \\
    \hspace{2mm}f-ANOVA & 0.6057 &  68.0000 &  8.5646 &     19.9519 &             3.0356 \\
    \hspace{2mm}GSS & 0.5749 &  87.4000 &  8.6319 &     26.0483 &             2.2070 \\
    \hspace{2mm}IG & 0.6194 &  84.8000 &  9.2644 &     29.1130 &             2.1274 \\
    \hspace{2mm}MI & 0.6031 &  84.2000 &  9.1788 &     28.3757 &             2.1255 \\
    \hspace{2mm}OR & 0.5502 & 150.2000 &  9.5490 &     54.7826 &             1.0043 \\
    \textbf{gender dataset}\\
    \hspace{2mm}CHI2 & 0.6417 & 293.0000 & 13.8191 &    223.8153 &             0.2867 \\
    \hspace{2mm}DE & 0.6442 &  41.8000 &  7.4090 &      9.1780 &             \textbf{7.0187} \\
    \hspace{2mm}ECE & 0.6321 & 365.6000 & 13.6071 &    270.7671 &             0.2334 \\
    \hspace{2mm}f-ANOVA & 0.6385 & 251.2000 & 12.5725 &    158.8265 &             0.4020 \\
    \hspace{2mm}GSS & 0.1892 &  53.0000 &  8.9622 &     17.0279 &             1.1109 \\
    \hspace{2mm}IG & 0.6427 & 284.2000 & 12.5812 &    179.9404 &             0.3572 \\
    \hspace{2mm}MI & 0.6411 & 292.4000 & 13.6436 &    217.7181 &             0.2945 \\
    \hspace{2mm}OR & 0.6364 & 337.6000 & 13.1601 &    233.8737 &             0.2721 \\
    \textbf{imdb dataset}\\
    \hspace{2mm}CHI2 & 0.6810 &  14.4000 &  6.3957 &      2.3561 &            \textbf{28.9034} \\
    \hspace{2mm}DE & 0.6966 &  17.0000 &  6.6829 &      3.0370 &            22.9384 \\
    \hspace{2mm}ECE & 0.4371 &  50.2000 &  8.8899 &     15.8692 &             2.7543 \\
    \hspace{2mm}f-ANOVA & 0.6840 &  16.4000 &  6.6628 &      2.9122 &            23.4883 \\
    \hspace{2mm}GSS & 0.5976 &  21.0000 &  7.2516 &      4.4172 &            13.5280 \\
    \hspace{2mm}IG & 0.6889 &  19.4000 &  7.1179 &      3.9315 &            17.5221 \\
    \hspace{2mm}MI & 0.6764 &  14.6000 &  6.4763 &      2.4494 &            27.6129 \\
    \hspace{2mm}OR & 0.5939 &  43.4000 &  8.9320 &     13.8499 &             4.2884 \\
    \textbf{tass dataset}\\
    \hspace{2mm}CHI2 & 0.4814 &  55.6000 &  8.5205 &     16.1460 &             2.9815 \\
    \hspace{2mm}DE & 0.3730 &  43.0000 &  7.7223 &     10.2572 &             \textbf{3.6366} \\
    \hspace{2mm}ECE & 0.2974 & 899.6000 & 14.7129 &    778.9390 &             0.0382 \\
    \hspace{2mm}f-ANOVA & 0.4533 &  57.6000 &  8.7544 &     17.6579 &             2.5673 \\
    \hspace{2mm}GSS & 0.4324 &  73.2000 &  9.0092 &     23.7654 &             1.8196 \\
    \hspace{2mm}IG & 0.4900 &  56.4000 &  8.6753 &     16.9789 &             2.8861 \\
    \hspace{2mm}MI & 0.4542 &  48.2000 &  8.6188 &     14.3219 &             3.1714 \\
    \hspace{2mm}OR & 0.3432 & 833.2000 & 14.4092 &    691.9755 &             0.0496 \\
    \bottomrule
    \end{tabular}
\end{table*}
